The Temporal Opportunist: Self-Supervised Multi-Frame Monocular Depth

Self-supervised monocular depth estimation networks are trained to predict scene depth using nearby frames as a supervision signal during training. However, for many applications, sequence information in the form of video frames is also available at test time. The vast majority of monocular networks do not make use of this extra signal, thus ignoring valuable information that could be used to improve the predicted depth. Those that do, either use computationally expensive test-time refinement techniques or off-the-shelf recurrent networks, which only indirectly make use of the geometric information that is inherently available. We propose ManyDepth, an adaptive approach to dense depth estimation that can make use of sequence information at test time, when it is available. Taking inspiration from multi-view stereo, we propose a deep end-to-end cost volume based approach that is trained using self-supervision only. We present a novel consistency loss that encourages the network to ignore the cost volume when it is deemed unreliable, e.g. in the case of moving objects, and an augmentation scheme to cope with static cameras. Our detailed experiments on both KITTI and Cityscapes show that we outperform all published self-supervised baselines, including those that use single or multiple frames at test time.

==> manydepth_arxiv 3/architecture_table.tex <==
\begin{tabular}[t]{|l|l|l|l|l|l|l|}
\hline
\textbf{layer} & \textbf{k} & \textbf{s} & \textbf{chns} & \textbf{res} & \textbf{input}   & \textbf{activation}    \\ \hline
\hline
\multicolumn{7}{|l|}{\textbf{Feature Extractor}} \\
\hline
conv1      &   7    &  2     &     64  &   2  &        image at time t             & ReLU  \\

max\_pool1      &       & 2     &       & 4   &        conv1              &   \\
resnet\_layer1      &       &       &     64  &   4  &        max\_pool1              &   \\ 

\hline
\multicolumn{7}{|l|}{} \\ \hline
\multicolumn{7}{|l|}{\textbf{Cost Volume}} \\
\hline
cost\_vol      &       &       &  96   & 4 &  resnet\_layer1 for t $\in \{0, -1\}$                        &   \\
conv\_reduce      &     3  &    1   & 64 &    4   &  resnet\_layer1\_t=0, cost\_vol &  ReLU                    \\


\hline
\multicolumn{7}{|l|}{} \\ \hline
\multicolumn{7}{|l|}{\textbf{Depth Decoder}} \\
\hline
%\textbf{layer} & \textbf{k} & \textbf{s} & \textbf{chns} & \textbf{res} & \textbf{input}   & \textbf{activation}    \\ \hline
resnet\_layer2      &       &       &     128  &   8  &       conv\_reduce              &   \\
resnet\_layer3      &       &       &     256  &   16  &        resnet\_layer2              &   \\
resnet\_layer4      &       &       &     512  &   32  &        resnet\_layer3              &   \\ \hline

upconv5       & 3      & 1      & 256      & 32    & resnet\_layer4                     & ELU \\
iconv5        & 3      & 1      & 256      & 16    & $\uparrow$upconv5, resnet\_layer3 & ELU \\ \hline

upconv4       & 3      & 1      & 128      & 16    & iconv5                    & ELU \\
iconv4        & 3      & 1      & 128      & 8     & $\uparrow$upconv4, resnet\_layer2 & ELU \\
disp4         & 3      & 1      & 1        & 1     & iconv4                    & Sigmoid \\ \hline

upconv3       & 3      & 1      & 64       & 8     & iconv4                    & ELU \\
iconv3        & 3      & 1      & 64       & 4     & $\uparrow$upconv3, resnet\_layer1 & ELU \\
disp3         & 3      & 1      & 1        & 1     & iconv3                   & Sigmoid  \\ \hline

upconv2       & 3      & 1      & 32       & 4     & iconv3                    & ELU \\
iconv2        & 3      & 1      & 32       & 2     & $\uparrow$upconv2, conv1 & ELU \\
disp2         & 3      & 1      & 1        & 1     & iconv2                    & Sigmoid \\ \hline

upconv1       & 3      & 1      & 16       & 2     & iconv2                    & ELU \\
iconv1        & 3      & 1      & 16       & 1     & $\uparrow$upconv1         & ELU \\
disp1         & 3      & 1      & 1        & 1     & iconv1                    & Sigmoid \\ \hline
% \multicolumn{7}{|l|}{} \\ \hline
% \multicolumn{7}{|l|}{\textbf{Pose Network}} \\
% \hline
% \textbf{layer} & \textbf{k} & \textbf{s} & \textbf{chns} & \textbf{res} & \textbf{input} & \textbf{activation}      \\ \hline
% pconv0         & 1      & 1      & 256      & 32     & econv5                    & ReLU \\ \hline
% pconv1         & 3      & 1      & 256      & 32     & pconv0 & ReLU\\ \hline %$\textrm{pconv0}_{t-1}$, $\textrm{pconv0}_{t}$, $\textrm{pconv0}_{t+1}$ \\ 
% pconv2         & 3      & 1      & 256      & 32    & pconv1                     & ReLU\\
% pconv3         & 1      & 1      & 6        & 32    & pconv3                     & - \\ \hline
% \multicolumn{6}{l}{} \\
% \hline
% \multicolumn{6}{|l|}{\textbf{Baseline pose network}} \\
% \hline
% \textbf{layer} & \textbf{k} & \textbf{s} & \textbf{chns} & \textbf{res} & \textbf{input}       \\ \hline
% pconv1         & 7      & 2      & 16      & 2      & $I_{t-1}$, $I_{t}$, $I_{t+1}$ \\ 
% pconv2         & 5      & 2      & 32      & 4      & pconv1                     \\
% pconv3         & 3      & 2      & 64      & 8      & pconv2                     \\ 
% pconv4         & 3      & 2      & 128     & 16     & pconv3                     \\ 
% pconv5         & 3      & 2      & 256     & 32     & pconv4                     \\ 
% pconv6         & 3      & 2      & 256     & 64     & pconv5                     \\ 
% pconv7         & 3      & 2      & 256     & 128    & pconv6                     \\ 
% pconv8         & 1      & 1      & 12      & 128    & pconv7                     \\ \hline
\end{tabular} 


==> manydepth_arxiv 3/main_results_table.tex <==
\newcommand{\x}{ x }
% \newcommand{\midline}{ \arrayrulecolor{gray}\hline }
\newcommand{\midline}{  }

% \newcommand{\splitline}{\arrayrulecolor{black}\cline{2-13}}
% \newcommand{\ssplitline}{\arrayrulecolor{black}\cline{3-13}}

\newcommand{\splitline}{\arrayrulecolor{black}\hhline{~------------}}
% \newcommand{\ssplitline}{\arrayrulecolor{black}\hhline{~------------}}

\newcommand*\rot{\rotatebox{90}}

\definecolor{Asectioncolor}{RGB}{255, 200, 200}
\definecolor{Bsectioncolor}{RGB}{255, 228, 196}
\definecolor{Csectioncolor}{RGB}{235, 255, 235}
\definecolor{Dsectioncolor}{RGB}{235, 235, 255}

% \setlength\arrayrulewidth{1pt} %Increasing linewidth 

\begin{table*}[t]
  \centering
  \footnotesize
  \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{|l|c|l|c|c|c||c|c|c|c|c|c|c|}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \arrayrulecolor{black}\hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
          &  TTR & Method & Test frames  & Semantics & WxH & \cellcolor{col1}Abs Rel & \cellcolor{col1}Sq Rel & \cellcolor{col1}RMSE  & \cellcolor{col1}RMSE log & \cellcolor{col2}$\delta < 1.25 $ & \cellcolor{col2}$\delta < 1.25^{2}$ & \cellcolor{col2}$\delta < 1.25^{3}$ \\
         
        \hline\hline
        \parbox[b]{2mm}{\multirow{16}{*}{\rotatebox[origin=c]{90}{Low and medium resolution}}} & 
        \cellcolor{Asectioncolor} & Ranjan \etal \cite{ranjan2018adversarial}  & 1 & & 832\x256 & 0.148 & 1.149 & 5.464 & 0.226 & 0.815 & 0.935 & 0.973\\
        \midline
        & \cellcolor{Asectioncolor} &  EPC++ \cite{luo2019every} & 1  && 832\x256 & 0.141 & 1.029 & 5.350 & 0.216 & 0.816 & 0.941 & 0.976\\
        \midline
        & \cellcolor{Asectioncolor}&  Struct2depth (M) \cite{casser2018depth}  & 1  &$\bullet$ &416\x128& 0.141 & {1.026} & 5.291 &  0.215 & 0.816 & 0.945 & {0.979}\\
        \midline
        & \cellcolor{Asectioncolor}&  Videos in the wild \cite{gordon2019depth} & 1 &$\bullet$ &  416\x128& 
        0.128 & 0.959  & 5.230 & 0.212 & 0.845 & 0.947 & 0.976 \\
        
        % & \cellcolor{Asectioncolor}&  Tosi \etal \cite{tosi2020distilled} & 1 &$\bullet$ &  640\x192& 
        % 0.126 &  0.835 & 4.937 & 0.199 & 0.844 &  0.953 &  0.982 \\
        
        \midline
        &  \cellcolor{Asectioncolor} &Guizilini \etal \cite{guizilini2020semantically} & 1 &$\bullet$ & 640\x192 & \underline{0.102} & \textbf{0.698} & \textbf{4.381} & \underline{0.178} & \underline{0.896} & \underline{0.964} & \textbf{0.984} \\
        \midline
        &  \cellcolor{Asectioncolor}& Johnston \etal~\cite{johnston2020self} & 1 && 640\x192 & 0.106 & 0.861 & 4.699 & 0.185 & 0.889 & 0.962 & 0.982 \\
        \midline
        &  \cellcolor{Asectioncolor}& Monodepth2 \cite{godard2019digging} & 1  &&  640\x192 &
         {0.115} &   {0.903} &   {4.863} &   {0.193} &   {0.877} &   {0.959} &   {0.981} \\ 
         \midline
        &  \cellcolor{Asectioncolor}& Packnet-SFM \cite{guizilini20203d} & 1 && 640\x192 & 0.111 & 0.785 & 4.601 & 0.189 & 0.878 & 0.960 & 0.982 \\
        \midline
        &  \cellcolor{Asectioncolor}& Li \etal \cite{li2020unsupervised}  & 1    & & 416\x128 &
        0.130 & 0.950 & 5.138 & 0.209 & 0.843 & 0.948 & 0.978 \\
        \midline
        &  \cellcolor{Asectioncolor}& Patil \etal \cite{patil2020dont}  & N    & & 640\x192  & 0.111  & 0.821  & 4.650  & 0.187  & 0.883  & 0.961  & 0.982 \\
        \midline
        &  \cellcolor{Asectioncolor}& Wang \etal \cite{wang2020self} & 2 (-1, 0)    & & 640\x192  & 0.106  & 0.799  & 4.662  & 0.187  & 0.889  & 0.961  & 0.982 \\
        \midline
        
        
        % \splitline
        
         & \cellcolor{Asectioncolor} &\textbf{ManyDepth (MR)} & 2 (-1, 0) & & 640\x192 &   \textbf{0.098}  &   \underline{0.770}  &   \underline{4.459}  &   \textbf{0.176}  &   \textbf{0.900}  &   \textbf{0.965}  &   \underline{0.983} \\
        
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \splitline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
        
         & $\bullet$  \cellcolor{Bsectioncolor} &GLNet \cite{chen2019self} & 3 (-1,  0, +1)   & & 416\x128  & 0.099  & 0.796  & 4.743  & 0.186  & 0.884  & 0.955  & 0.979 \\
        \midline
        & $\bullet$  \cellcolor{Bsectioncolor} &Luo \etal \cite{luo2020consistent} & N && 384\x112 &  0.130 &  2.086 & 4.876 & 0.205 & 0.878 & 0.946 &  0.970\\
        \midline
        & $\bullet$ \cellcolor{Bsectioncolor} & CoMoDA \cite{kuznietsov2021comoda} &  N & $\bullet$ &  640\x192 & 0.103 & 0.862 & 4.594 &  0.183  & 0.899 &  0.961 &  0.981 \\
        
        
        \midline
         & $\bullet$ \cellcolor{Bsectioncolor} &McCraith \etal \cite{mccraith2020monocular} & 2 (0, +1)&& 640\x192 & \textbf{0.089} & \underline{0.747} & \underline{4.275}  & \underline{0.173} & \underline{0.912} & \underline{0.964} & \underline{0.982} \\
        \midline
        & $\bullet$ \cellcolor{Bsectioncolor} & Struct2depth (M+R) \cite{casser2018depth}  &  3 (-1,  0,  +1)       &$\bullet$  & 416\x128  & 0.109  & 0.825  & 4.750  & 0.187  & 0.874  & 0.958  & \textbf{0.983} \\
        % \splitline
        & $\bullet$ \cellcolor{Bsectioncolor} & \textbf{{ManyDepth (MR + TTR)}} & 2 (-1, 0) & & 640\x192 &   \underline{0.090}  &   \textbf{0.713}  &   \textbf{4.261}  &   \textbf{0.170}  &   \textbf{0.914}  &   \textbf{0.966}  &   \textbf{0.983} \\
            
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \arrayrulecolor{black}\hline\hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                
        \parbox[b]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{High resolution}}} 
        & \cellcolor{Csectioncolor} &Monodepth2 \cite{godard2019digging}   & 1 &  & 1024\x320 &
         {0.115} &   {0.882} &   {4.701} &   {0.190} &   {0.879} &   {0.961} &   {0.982} \\ 
        \midline
         &\cellcolor{Csectioncolor}& Packnet-SFM \cite{guizilini20203d} & 1 &&  1280\x384 &  0.107 & 0.802 & 4.538 & 0.186 & 0.889 & 0.962 & 0.981 \\
         \midline
         & \cellcolor{Csectioncolor}& Guizilini \etal \cite{guizilini2020semantically} & 1 &$\bullet$ & 1280\x384 & 0.100 & 0.761 & 4.270 & 0.175 & 0.902 & 0.965 & 0.982 \\
        %  & \cellcolor{Csectioncolor}&  Tosi \etal \cite{tosi2020distilled} & 1 &$\bullet$ &  1024\x320 &  
        %  0.125 & 0.805 & 4.795 & 0.195 & 0.849 & 0.955 & 0.983 \\
         \midline
         &  \cellcolor{Csectioncolor}& Shu \etal~\cite{shu2020feature} (ResNet50) & 1 && 1024\x320 & 0.104 & 0.729 & 4.481 & 0.179 & 0.893 & 0.965 & \textbf{0.984} \\
         \midline
        & \cellcolor{Csectioncolor} &Wang \etal \cite{wang2020self} & 2 (-1, 0)    & & 1024\x320  & 0.106  & 0.773  & 4.491  & 0.185  & 0.890  & 0.962  & 0.982 \\
        \midline
        
        % Wang \etal $^*$ \cite{wang2019recurrent} & 10 (-9, ..., 0)    & & 416\x128  & \sout{0.112}  & \sout{0.418}  & \sout{2.32}  & \sout{0.153}  & \sout{0.882}  & \sout{0.974}  & \sout{0.992} \\  
        
        
        % \splitline
        
        & \cellcolor{Csectioncolor}& \textbf{ManyDepth (HR)} & 2 (-1, 0) && 1024\x320 &   \underline{0.093}  &   \underline{0.715}  &   \textbf{4.245}  &   \underline{0.172}  &   \underline{0.909}  &   \underline{0.966}  &   \underline{0.983}  \\
        
        \midline
        
        & \cellcolor{Csectioncolor} & \textbf{ManyDepth (HR ResNet50)} & 2 (-1, 0) && 1024\x320 &    \textbf{0.091}  &   \textbf{0.694}  &   \textbf{4.245}  &   \textbf{0.171}  &   \textbf{0.911}  &   \textbf{0.968}  &   \underline{0.983}  \\
        
        \splitline %\splitline
        
        
        & $\bullet$ \cellcolor{Dsectioncolor} & McCraith \etal \cite{mccraith2020monocular} & 2 (0, +1)  & & 1024\x320 & 0.089 & 0.756 & 4.228 & 0.170 & 0.917 & 0.967 & \textbf{0.983} \\
        
        \midline
        & $\bullet$ \cellcolor{Dsectioncolor} &Shu \etal~\cite{shu2020feature}  (ResNet50) & 3 (-1, 0, +1)  &  & 1024\x320 & 0.088 &  0.712 & \textbf{4.137} & 0.169 & 0.915 & 0.965 & 0.982 \\
        
        \midline
        
        & $\bullet$ \cellcolor{Dsectioncolor} &\textbf{ManyDepth (HR + TTR)} & 2 (-1, 0) && 1024\x320 &   \textbf{0.087}  &   \underline{0.696}  &   4.183  &   \textbf{0.167}  &   \underline{0.918}  &   \textbf{0.968}  &   \textbf{0.983}  \\
        
        & $\bullet$ \cellcolor{Dsectioncolor} &\textbf{ManyDepth (HR R50 + TTR)} & 2 (-1, 0) && 1024\x320 &   \textbf{0.087}  &   \textbf{0.685}  &   \underline{4.142}  &   \textbf{0.167}  &   \textbf{0.920}  &   \textbf{0.968}  &   \textbf{0.983}  \\

        
        \arrayrulecolor{black}\hline

    \end{tabular}
  }  % end resizebox
  \vspace{-1pt}
  \caption{\textbf{Comparison of our method to existing self-supervised approaches on the KITTI~\cite{Geiger2012CVPR} Eigen split.}   
At the top we compare medium and low resolution results {\setlength{\fboxsep}{0pt}\colorbox{Asectioncolor}{without}}  and {\setlength{\fboxsep}{0pt}\colorbox{Bsectioncolor}{with}} test-time refinement (TTR).
  At bottom we compare high resolution results {\setlength{\fboxsep}{0pt}\colorbox{Csectioncolor}{without}}  and {\setlength{\fboxsep}{0pt}\colorbox{Dsectioncolor}{with}} TTR. 
   The best results in each subsection are in \textbf{bold}; second best are \underline{underlined}.
%   At top we compare medium and low resolution results \colorbox{Asectioncolor}{without}  and \colorbox{Bsectioncolor}{with} test-time refinement (TTR).
%   At bottom we compare high resolution results \colorbox{Csectioncolor}{without}  and \colorbox{Dsectioncolor}{with} TTR. 
%   Best results in each subsection are in \textbf{bold}; second best are \underline{underlined}.
   Our method outperforms all previous methods in all subsections across most metrics, whether or not the baselines use multiple frames at test time. 
   We indicate if a method uses semantic supervision (Semantics) and methods indicated by N take a long sequence of frames as input for each test image (\eg the preceding frames or frames before and after in time).
%   or if it is evaluated on whole sequences ($^\dagger$) rather than sets of two or three frames. 
%   \oma{Can we clarify in a few words what `whole sequences' means? } 
%   \oma{I like the colorful TTR column, but I'm not sure it is necessary to color it.}
   % {  % start legend
%         \footnotesize
%         \newline
%         \textbf{Legend:} \hspace{10pt} 
%         TTR -- Uses test-time refinement \hspace{10pt}
%         Semantics -- Semantic supervision \hspace{10pt}
%         $^\dagger$ -- Evaluated on whole sequences
%     } % end legend
    \label{tab:kitti_eigen}} % end caption
    
    \vspace{-5pt}


\end{table*}

  %Comparison of our method to existing methods, all trained on monocular sequences from KITTI 2015 \cite{Geiger2012CVPR} using the Eigen split and evaluated on the KITTI 2015 test set.



% \newline
% $^*$ Wang \etal probably evaluated on new ground truth. Some suspicions around the evaluation too, \eg train/test split; see their github issues.






% OLD



% \cite{gonzalez2020forget}  &  \\
% Garg \cite{garg2016unsupervised}\te\xtdagger & 1 &  K  & S &&  0.152 & 1.226 & 5.849 & 0.246 & 0.784 & 0.921 & 0.967\\
% Monodepth R50 \cite{godard2017unsupervised}\te\xtdagger & 1 &  K & S && 0.133 & 1.142 & 5.533 & 0.230 & 0.830 & 0.936 & 0.970\\
% StrAT \cite{mehta2018structured}  & 1  & K  & S &&  0.128 & 1.019 & 5.403 & 0.227 & 0.827 & 0.935 & 0.971\\
% 3Net  (R50) \cite{poggi20183net} & 1 &  K & S && 0.129 & 0.996 & 5.281 & 0.223 & 0.831 & 0.939 & 0.974 \\
% 3Net (VGG)  \cite{poggi20183net} & 1 &  K & S && 0.119 &  1.201 & 5.888 & 0.208 &  0.844 & 0.941 & \te\xtbf{0.978}  \\
% SuperDepth + pp \cite{pillai2018superdepth}  & 1  & K & S & 1024 $\times$ 382 & \underline{0.112} & \underline{0.875} & \te\xtbf{4.958} & \te\xtbf{0.207} & \underline{0.852} & \underline{0.947} & \underline{0.977} \\


% % {\bf Monodepth2} w/o pretraining &&  S  &&&   
% % 0.130 &   1.144 &   5.485 &   0.232 &   0.831 &   0.932 &   0.968 \\ 
% {\bf Monodepth2}      &  1    &      K & S && 
% \te\xtbf{0.109} &   \te\xtbf{0.873} &   \underline{4.960} &   \underline{0.209} &   \te\xtbf{0.864} &   \te\xtbf{0.948} &   0.975 \\ 
% \arrayrulecolor{gray}\hline

% {\bf Monodepth2} & 1 &    K & S & 1024 $\times$ 320 & 
%   \te\xtbf{0.107} &   \te\xtbf{0.849} &   \te\xtbf{4.764} &   \te\xtbf{0.201} &   \te\xtbf{0.874} &   \te\xtbf{0.953} &   \underline{0.977} \\ 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \arrayrulecolor{black}\hline
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% UnDeepVO \cite{li2018undeepvo} & 1 &  K  & MS &&  0.183 & 1.730 & 6.57 & 0.268 & - & - & -\\
% Zhan FullNYU \cite{zhanst2018} & 1 &  K  & D*MS &&  0.135 & 1.132 & 5.585 & 0.229 & 0.820 & 0.933 & 0.971\\
% EPC++ \cite{luo2018every} &  1 & K & MS && 0.128 & \underline{0.935} & \underline{5.011} & \underline{0.209} & 0.831 & \underline{0.945} & \te\xtbf{0.979} \\
% %   \te\xtbf{Monodepth2} w/o pretraining &&  MS &&&   
% %   \underline{0.127} &   1.031 &   5.266 &   0.221 &   \underline{0.836} &   0.943 &   \underline{0.974} \\
% \te\xtbf{Monodepth2} &  1 & K  & MS  &&
%   \te\xtbf{0.106} &   \te\xtbf{0.818} &   \te\xtbf{4.750} &   \te\xtbf{0.196} &   \te\xtbf{0.874} &   \te\xtbf{0.957} &   \te\xtbf{0.979} \\

%   \arrayrulecolor{gray}\hline
%   \te\xtbf{Monodepth2}  & 1  & K & MS & 1024 $\times$ 320
%     &   \te\xtbf{0.106} &   \te\xtbf{0.806} &   \te\xtbf{4.630} &   \te\xtbf{0.193} &   \te\xtbf{0.876} &   \te\xtbf{0.958} &   \te\xtbf{0.980}  \\
    
%   \hline
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% &   & K  & MS  & 192\x640  & 0.102  & 0.776  & 4.534  & 0.183  & 0.893  & 0.963  & 0.982 \\
%   &   & K  & MS  & 320\x1024  & 0.101  & 0.725  & 4.36  & 0.179  & 0.898  & 0.965  & 0.983 \\
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \te\xtbf{Lidar supervision} \\  
% SVSM FT \cite{singlestereo2018} & 1  &DS && \underline{0.094} & \underline{0.626} & 4.252 & 0.177 & 0.891 & 0.965 & 0.984\\
% Guo \cite{guo2018learning} & 1 & DS & & 0.096 & 0.641  & \underline{4.095}  & \underline{0.168}  & \underline{0.892}  & \underline{0.967}  & \underline{0.986} \\
% DORN \cite{fu2018deep}\ddag & 1 &  D & &  0.098  &   0.581  &   3.666  &   0.160  &   0.899  &   0.967  &  0.986 \\
% %  \sout{0.072}&  \sout{0.307} & \sout{2.727} & \sout{0.120} & \sout{0.932} & \sout{0.984} & \sout{0.994}\\ 
% Kumar \etal \cite{kumar2018depthnet} & 3 (-2, -1, 0) &  D  & ?  & 0.137  & 1.019  & 5.187  & 0.218  & 0.809  & 0.928  & 0.971 \\
% \hline
%   Eom \etal \cite{eom2019temporally} &   & DM  & ?  & 0.117  & 0.726  & 4.537  & 0.192  & 0.865  & 0.958  & 0.983 \\
%   Patil \etal \cite{patil2020dont}  & N$^\dagger$    & D  & 640\x192  & 0.102  & 0.655  & 4.148  & 0.172  & 0.884  & 0.966  & 0.987 \\
%   Wang \etal $^*$ \cite{wang2019recurrent} & 10 (-9, ..., 0)    & D  & 416\x128  & \sout{0.077}  & \sout{0.205}  & \sout{1.698}  & \sout{0.11}  & \sout{0.941}  & \sout{0.99}  & \sout{0.998} \\
  
% These results are not Eigen Neural RGB$\rightarrow$D \cite{liu2019neural} & N$^\dagger$ ?? &  D+GPS/IMU & 1248\x 380? &  0.0998 & 0.473 &  2.829 & 0.128 & 0.932 & 0.980 & 0.993 \\ 
% % image size from https://github.com/NVlabs/neuralrgbd/blob/master/code/mdataloader/kitti.py
% These results are not Eigen Neural RGB$\rightarrow$D \cite{liu2019neural} & N$^\dagger$?? &  D & 1248\x 380? &  0.120 & 0.576 & 3.516 & 0.167  & 0.878 & 0.972 & 0.991 \\ 
    
    
    
    
    
    
% \begin{table*}
%   \centering
%     % \begin{minipage}[l]{1.0\textwidth}
%   \resizebox{1.0\textwidth}{!}{
%   \begin{tabular}{|c|l|c|c||c|c|c|c|c|c|c|}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \arrayrulecolor{black}\hline
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% & Method & Test frames &  WxH & \cellcolor{col1}Abs Rel & \cellcolor{col1}Sq Rel & \cellcolor{col1}RMSE  & \cellcolor{col1}RMSE log & \cellcolor{col2}$\delta < 1.25 $ & \cellcolor{col2}$\delta < 1.25^{2}$ & \cellcolor{col2}$\delta < 1.25^{3}$ \\
%   \hline
% \arrayrulecolor{black}\hline\arrayrulecolor{gray}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \multirow{3}{2cm}{Semantic \\ supervision} & Struct2Depth 2 \cite{Casser_2019_CVPR_Workshops}  &  1  &   416\x128 &  0.145  & 1.737  & 7.280  &  0.205 & 0.813 & 0.942 & 0.976 \\
% \splitline
% & Struct2Depth 2 \cite{Casser_2019_CVPR_Workshops}  &  3 (-1,  0,  +1)  & 416\x128 &  
% 0.151 & 2.492 & 7.024 & 0.202 & 0.826 & 0.937 & 0.972 \\
% \splitline
% & Videos in the Wild \cite{gordon2019depth} & 1 & 416\x128 & 
% \textbf{0.127} & \textbf{1.330} & \textbf{6.960} & \textbf{0.195} & \textbf{0.830} & \textbf{0.947} & \textbf{0.981} \\

% \arrayrulecolor{black}\hline\hline
% % \arrayrulecolor{black}\hline\arrayrulecolor{gray}
% \multirow{4}{*}{No semantics} & Monodepth2$\dagger$ \cite{godard2019digging} & 1  & 512\x192 &  
% 0.154  &   1.840  &   7.774  &   0.216  &   0.792  &   0.945  &   0.981 \\
% \splitline
% & Pilzer \etal \cite{pilzer2018unsupervised} & 1 & 512\x256 & 
% 0.440 & 6.036 & \textbf{5.443} & 0.398 & 0.730 & 0.887 & 0.944 \\
% \splitline
% & Struct2Depth 2 \cite{Casser_2019_CVPR_Workshops}  &  3 (-1,  0,  +1)    & 416\x128 &  
% 0.222  & 5.737  & 8.613  & 0.258  & 0.774  & 0.908 & 0.954 \\
% \splitline
% % ManyDepth & 2 (-1, 0) & M & 192x640 & 0.150  &   1.798  &   7.589  &   0.208  &   0.814  &   0.948  &   0.982 \\
% % ManyDepth & & & &   0.144  &   1.659  &   7.266  &   0.201  &   0.823  &   0.954  &   0.984 \\
% & {\bf ManyDepth} & 2 (-1, 0)  & 512\x192 &   
% \textbf{0.114}  &   1.193  &   6.223  &   0.170  &   0.875  &   0.967  &   0.989 \\
% % \textbf{0.139}  &   \textbf{1.633}  &   7.331  &   \textbf{0.199}  &   \textbf{0.826}  &   \textbf{0.953}  &   \textbf{0.984}  \\


    
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \arrayrulecolor{black}\hline
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   \end{tabular}
%   }
%   \vspace{-2pt}
%   \caption{\textbf{Results on Cityscapes.} 
%   Results in the top section use semantic supervision, which is especially beneficial on this dataset with many moving objects. Our method beats all non-semantically-trained models, and even rivals baselines with semantic supervision. $\dagger$ is trained by us using the authors' code, with the data preprocessing from \cite{zhou2017unsupervised}. \label{tab:cs_train_test}}
%   \vspace{-5pt}
% \end{table*}


==> manydepth_arxiv 3/results_fig.tex <==
\newcommand{\turnwidthnew}{0.6\columnwidth}

\hspace{-10pt}
\centering

%images are 347 632 222 and 474

\newcommand{\imlabel}[2]{\includegraphics[width=\turnwidthnew]{#1}%
\raisebox{35pt}{\makebox[2pt][r]{\small #2}}}

% \raisebox{10pt}{#2}}


\begin{tabular}{@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 2mm}c@{}}
% & Input & Monodepth2 \cite{godard2019digging} &  Don't forget the past \cite{patil2020dont} & Ours (mono) & Ours (multi) \\

{\rotatebox{90}{\hspace{1mm}\footnotesize Input \& GT}} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/colors/688_color.jpg} &
% \includegraphics[width=\turnwidthnew]{figs/main_fig/lidar/643.jpg} &
\imlabel{figs/main_fig/lidar/643.jpg}{Ground truth depth} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/colors/478_color.jpg} &
% \includegraphics[width=\turnwidthnew]{figs/main_fig/lidar/444.jpg} \\
\imlabel{figs/main_fig/lidar/444.jpg}{Ground truth depth} \\


{\rotatebox{90}{\hspace{4mm}\footnotesize \cite{godard2019digging} MR}} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/mdp2_LR_disp/643.jpg} &
\imlabel{figs/main_fig//mdp2_LR_error/643.jpg}{Error map} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/mdp2_LR_disp/444.jpg} &
\imlabel{figs/main_fig//mdp2_LR_error/444.jpg}{Error map}  \\

{\rotatebox{90}{\hspace{4mm} \cite{guizilini20203d}}} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/packnet_LR_disp/643.jpg} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/packnet_LR_error/643.jpg} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/packnet_LR_disp/444.jpg} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/packnet_LR_error/444.jpg}\\

{\rotatebox{90}{\hspace{4mm}\cite{patil2020dont}}} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/DFTP_disp/643.jpg} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/DFTP_error/643.jpg} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/DFTP_disp/444.jpg} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/DFTP_error/444.jpg}\\

{\rotatebox{90}{\hspace{2mm}\footnotesize Ours MR}} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/ours_LR_disp/643.jpg} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/ours_LR_error/643.jpg} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/ours_LR_disp/444.jpg} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/ours_LR_error/444.jpg}\\

{\rotatebox{90}{\hspace{1mm}\footnotesize Ours + TTR}} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/refined_oursLR_disps/643_disp.jpg} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/refined_oursLR_error/643_error.jpg} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/refined_oursLR_disps/444_disp.jpg} &
\includegraphics[width=\turnwidthnew]{figs/main_fig/refined_oursLR_error/444_error.jpg}\\



\end{tabular}


==> manydepth_arxiv 3/results_table_new_ground_truth.tex <==

% \newcommand{\midline}{ \arrayrulecolor{gray}\hline }
\renewcommand{\midline}{  }

% \newcommand{\splitline}{\arrayrulecolor{black}\cline{2-13}}
% \newcommand{\ssplitline}{\arrayrulecolor{black}\cline{3-13}}

\renewcommand{\splitline}{\arrayrulecolor{black}\hhline{~------------}}
% \newcommand{\ssplitline}{\arrayrulecolor{black}\hhline{~------------}}

\renewcommand*\rot{\rotatebox{90}}

\definecolor{Asectioncolor}{RGB}{255, 200, 200}
\definecolor{Bsectioncolor}{RGB}{255, 228, 196}
\definecolor{Csectioncolor}{RGB}{235, 255, 235}
\definecolor{Dsectioncolor}{RGB}{235, 235, 255}

% \setlength\arrayrulewidth{1pt} %Increasing linewidth 

\begin{table*}[t]
  \centering
  \footnotesize
  \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{|l|c|l|c|c|c||c|c|c|c|c|c|c|}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \arrayrulecolor{black}\hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
          &  TTR & Method & Test frames  & Semantics & WxH & \cellcolor{col1}Abs Rel & \cellcolor{col1}Sq Rel & \cellcolor{col1}RMSE  & \cellcolor{col1}RMSE log & \cellcolor{col2}$\delta < 1.25 $ & \cellcolor{col2}$\delta < 1.25^{2}$ & \cellcolor{col2}$\delta < 1.25^{3}$ \\
         
        \hline\hline
        \parbox[b]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{LR + MR}}} & 
        \cellcolor{Asectioncolor} & Ranjan \cite{ranjan2018adversarial}  & 1 & & 832\x256  &
        0.123 & 0.881 & 4.834 & 0.181 & 0.860 & 0.959 & 0.985\\
        \midline
        & \cellcolor{Asectioncolor} &  EPC++ \cite{luo2019every} & 1  && 832\x256 & 
        0.120 & 0.789 &  4.755  & 0.177  & 0.856 &  0.961 &  0.987\\
        \midline

        % \midline
        &  \cellcolor{Asectioncolor}& Johnston \etal~\cite{johnston2020self} & 1 && 640\x192 &
        0.081 & 0.484  & 3.716  & 0.126  & 0.927  & 0.985  & 0.996 \\
        \midline
        &  \cellcolor{Asectioncolor}& Monodepth2 \cite{godard2019digging} & 1  &&  640\x192 &
         0.090 & 0.545 & 3.942 & 0.137 & 0.914 & 0.983 & 0.995
        \\ 
         \midline
        &  \cellcolor{Asectioncolor}& Packnet-SFM \cite{guizilini20203d} & 1 && 640\x192 &
         0.078 & 0.420 &  3.485 &  0.121 &  0.931 &  0.986 &  0.996
         \\
        \midline
        &  \cellcolor{Asectioncolor}& Patil \etal \cite{patil2020dont}  & N$^\dagger$    & & 640\x192 
        &   0.087  &   0.495  &   3.775  &   0.133  &   0.917  &   0.983  &   0.995  \\
        
        \midline
        &  \cellcolor{Asectioncolor}& Wang \etal \cite{wang2020self} & 2 (-1, 0)    & & 640\x192  & 
        0.082 & 0.462 & 3.739 & 0.127 &  0.923 &  0.984 & 0.996\\
        \midline
        
        
        
        % \splitline
        
         & \cellcolor{Asectioncolor} &\textbf{ManyDepth (MR)} & 2 (-1, 0) & & 640\x192 &  \textbf{0.070}  &   \textbf{0.399}  &   \textbf{3.455}  &   \textbf{0.113}  &   \textbf{0.941}  &   \textbf{0.989}  &   \textbf{0.997}\\
        
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \splitline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
        
        % \splitline
        & $\bullet$ \cellcolor{Bsectioncolor} & \textbf{{ManyDepth (MR + TTR)}} & 2 (-1, 0) & & 640\x192 & \textbf{0.058}  &   \textbf{0.334}  &   \textbf{3.137}  &   \textbf{0.101}  &   \textbf{0.958}  &   \textbf{0.991}  &   \textbf{0.997} \\
            
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \arrayrulecolor{black}\hline\hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                
        \parbox[b]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{HR}}} 
        & \cellcolor{Csectioncolor} &Monodepth2 \cite{godard2019digging}   & 1 &  & 1024\x320 &  0.091  &   0.531  &   3.742  &   0.135  &   0.916  &   0.984  &   0.995  \\
        % \midline

        
        
        \midline
        
        & \cellcolor{Csectioncolor}& \textbf{ManyDepth (HR)} & 2 (-1, 0) && 1024\x320 & 0.064  &   0.345  &   \textbf{3.116}  &   0.103  &   0.949  &   0.989  &   \textbf{0.997}  \\
        
        \midline
        
        & \cellcolor{Csectioncolor} & \textbf{ManyDepth (HR ResNet50)} & 2 (-1, 0) && 1024\x320 &   \textbf{0.062}  &   \textbf{0.343}  &   3.139  &   \textbf{0.102}  &   \textbf{0.953}  &   \textbf{0.991}  &   \textbf{0.997} \\
        
        
        \splitline
        
        & $\bullet$ \cellcolor{Dsectioncolor} &\textbf{ManyDepth (HR + TTR)} & 2 (-1, 0) && 1024\x320 &   0.056  &   0.322  &   3.034  &   0.096  &   0.961  &   0.992  &   0.997 \\
        
        & $\bullet$ \cellcolor{Dsectioncolor} &\textbf{ManyDepth (HR ResNet50 + TTR)} & 2 (-1, 0) && 1024\x320 &   \textbf{0.055}  &   \textbf{0.305}  &   \textbf{2.945}  &   \textbf{0.094}  &   \textbf{0.963}  &  \textbf{ 0.992}  &   \textbf{0.997} \\

        
        \arrayrulecolor{black}\hline

    \end{tabular}
  }  % end resizebox
  \vspace{-1pt}
  \caption{\textbf{KITTI~\cite{Geiger2012CVPR} evaluation on improved ground truth from \cite{uhrig2017sparse}, as described in \cite{godard2019digging}.}   As in the main paper, at top we compare medium and low resolution results \colorbox{Asectioncolor}{without}  and \colorbox{Bsectioncolor}{with} test-time refinement (TTR).
  At bottom we compare high resolution results \colorbox{Csectioncolor}{without}  and \colorbox{Dsectioncolor}{with} TTR.
   Best results in each subsection are in \textbf{bold}.
  Our method outperforms all previous methods in all subsections across all metrics, whether or not the baselines use multiple frames at test time.
  We don't report results on the new ground truth using the methods \cite{mccraith2020monocular, casser2018depth, Casser_2019_CVPR_Workshops, gordon2019depth, guizilini2020semantically, chen2019self, luo2020consistent, shu2020feature} as they were not reported in the publications, and the raw predictions have not been made public by the authors. None of the methods presented here were trained with semantics.
  {  % start legend
        \footnotesize
        \newline
        \textbf{Legend:} \hspace{10pt} 
        TTR -- Uses test-time refinement \hspace{10pt}
        Semantics -- Semantic supervision \hspace{10pt}
        $^\dagger$ -- evaluated on whole sequences
    } % end legend
    \label{tab:kitti_improved_ground_truth}} % end caption
    
    \vspace{-5pt}


\end{table*}

==> manydepth_arxiv 3/sup_results_fig.tex <==
\newcommand{\turnheightnew}{0.195\columnwidth}
\newcommand{\turnwidthnew}{0.8\columnwidth}

\centering

%images are 347 632 222 and 474

\newcommand{\imlabel}[2]{\includegraphics[width=\turnwidthnew]{#1}%
\raisebox{35pt}{\makebox[2pt][r]{\small #2}}}

% \raisebox{10pt}{#2}}



\begin{figure*}
  \centering
    % \begin{minipage}[l]{1.0\textwidth}
  \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{m{3.5cm}m{6cm}m{6cm}}
        
        % & Input & Monodepth2 Monodepth2 \cite{godard2019digging} &  Don't forget the past \cite{patil2020dont} & Ours (mono) & Ours (multi) \\
        Input and ground truth &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/463_color.jpg} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/463_gt_disp.jpg} \\
        ManyDepth (MR) &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/463_ours_LR_disp.jpg} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/463_ours_LR_error.jpg} \\
        Monodepth2 \cite{godard2019digging} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/463_mdp2_LR_disp.jpg} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/463_mdp2_LR_error.jpg} \\
        DFTP \cite{patil2020dont} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/463_DFTP_disp.jpg} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/463_DFTP_error.jpg} \\
        Packnet-SFM \cite{guizilini20203d} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/463_packnet_LR_disp.jpg} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/463_packnet_LR_error.jpg} \\
        
        Input and ground truth &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/328_color.jpg} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/328_gt_disp.jpg} \\
        ManyDepth (MR) &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/328_ours_LR_disp.jpg} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/328_ours_LR_error.jpg} \\
        Monodepth2 \cite{godard2019digging} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/328_mdp2_LR_disp.jpg} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/328_mdp2_LR_error.jpg} \\
        DFTP \cite{patil2020dont} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/328_DFTP_disp.jpg} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/328_DFTP_error.jpg} \\
        Packnet-SFM \cite{guizilini20203d} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/328_packnet_LR_disp.jpg} &
        \includegraphics[width=\turnwidthnew]{sup_results_fig/328_packnet_LR_error.jpg} \\
    \end{tabular}
    }
    \caption{\textbf{Further qualitative results on the KITTI dataset (part 1)}. Error maps on the right measure the absolute relative error compared to the ground truth, after median scaling \cite{eigen2015predicting}. Errors range from blue (low error, abs.~rel.~$=0.0$) to red (high error, abs.~rel.~$=0.2$). The color mapping in all error maps are the same, and the colorbar is shown in Figure~\ref{fig:colormap}. \label{fig:extra_kitti_qual_1}}
    
\end{figure*}


\begin{figure*}
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{m{3.5cm}m{6cm}m{6cm}}
    
            
            Input and ground truth &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/146_color.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/146_gt_disp.jpg} \\
            ManyDepth (MR) &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/146_ours_LR_disp.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/146_ours_LR_error.jpg} \\
            Monodepth2 \cite{godard2019digging} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/146_mdp2_LR_disp.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/146_mdp2_LR_error.jpg} \\
            DFTP \cite{patil2020dont} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/146_DFTP_disp.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/146_DFTP_error.jpg} \\
            Packnet-SFM \cite{guizilini20203d} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/146_packnet_LR_disp.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/146_packnet_LR_error.jpg} \\
            
            Input and ground truth &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/052_color.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/052_gt_disp.jpg} \\
            ManyDepth (MR) &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/052_ours_LR_disp.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/052_ours_LR_error.jpg} \\
            Monodepth2 \cite{godard2019digging} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/052_mdp2_LR_disp.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/052_mdp2_LR_error.jpg} \\
            DFTP \cite{patil2020dont} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/052_DFTP_disp.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/052_DFTP_error.jpg} \\
            Packnet-SFM \cite{guizilini20203d} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/052_packnet_LR_disp.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/052_packnet_LR_error.jpg} \\
            
    

        \end{tabular}
        }
        \caption{\textbf{Further qualitative results on the KITTI dataset (part 2)}. Error maps on the right measure the absolute relative error compared to the ground truth, after median scaling \cite{eigen2015predicting}. Errors range from blue (low error, abs.~rel.~$=0.0$) to red (high error, abs.~rel.~$=0.2$). The color mapping in all error maps are the same, and the colorbar is shown in Figure~\ref{fig:colormap}. \label{fig:extra_kitti_qual_2}}
\end{figure*}
    


\begin{figure*}
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{m{3.5cm}m{6cm}m{6cm}}
    
            

            Input and ground truth &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/643_color.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/643_gt_disp.jpg} \\
            ManyDepth (MR) &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/643_ours_LR_disp.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/643_ours_LR_error.jpg} \\
            Monodepth2 \cite{godard2019digging} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/643_mdp2_LR_disp.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/643_mdp2_LR_error.jpg} \\
            DFTP \cite{patil2020dont} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/643_DFTP_disp.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/643_DFTP_error.jpg} \\
            Packnet-SFM \cite{guizilini20203d} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/643_packnet_LR_disp.jpg} &
            \includegraphics[width=\turnwidthnew]{sup_results_fig/643_packnet_LR_error.jpg} \\
    
        \end{tabular}
        }
        \caption{\textbf{Further qualitative results on the KITTI dataset (part 3)}. Error maps on the right measure the absolute relative error compared to the ground truth, after median scaling \cite{eigen2015predicting}. Errors range from blue (low error, abs.~rel.~$=0.0$) to red (high error, abs.~rel.~$=0.2$). The color mapping in all error maps are the same, and the colorbar is shown in Figure~\ref{fig:colormap}.  \label{fig:extra_kitti_qual_3}}
\end{figure*}


==> manydepth_arxiv 3/wander_results_fig.tex <==


%images are 347 632 222 and 474

% \raisebox{10pt}{#2}}
\newcommand{\itemwidth}{0.35\columnwidth}


\begin{figure*}
  \centering
    % \begin{minipage}[l]{1.0\textwidth}
  \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 2mm}c@{}}
        
        {\scriptsize Input} &  {\scriptsize ManyDepth} & {\scriptsize Monodepth2 \cite{godard2019digging}} \\
        % & Ours (multi) \\
        \includegraphics[width=\itemwidth]{wander_fig/000_color.jpg} &
        \includegraphics[width=\itemwidth]{wander_fig/000_multi_circles.png} &
        \includegraphics[width=\itemwidth]{wander_fig/000_mono.jpg} \\
        
        \includegraphics[width=\itemwidth]{wander_fig/015_color.jpg} &
        \includegraphics[width=\itemwidth]{wander_fig/015_multi_circles.png} &
        \includegraphics[width=\itemwidth]{wander_fig/015_mono.jpg} \\
        
        \includegraphics[width=\itemwidth]{wander_fig/034_color.jpg} &
        \includegraphics[width=\itemwidth]{wander_fig/034_multi_circles.png} &
        \includegraphics[width=\itemwidth]{wander_fig/034_mono.jpg} \\
        
        \includegraphics[width=\itemwidth]{wander_fig/050_color.jpg} &
        \includegraphics[width=\itemwidth]{wander_fig/050_multi_circles.png} &
        \includegraphics[width=\itemwidth]{wander_fig/050_mono.jpg} \\
        
        \includegraphics[width=\itemwidth]{wander_fig/093_color.jpg} &
        \includegraphics[width=\itemwidth]{wander_fig/093_multi_circles.png} &
        \includegraphics[width=\itemwidth]{wander_fig/093_mono.jpg} \\
        
    \end{tabular}
    }
    \caption{\textbf{Qualitative results on YouTube videos}. All predictions are made with a model trained on the KITTI dataset. Note how our method is able to correctly estimate the shape of the sign in the top row, the car on the left in the second row, the pillars in the third row, and the signs in the fourth and fifth rows. \label{fig:wander}}
    
\end{figure*}


